Superflows: A New Tool for Forensic Network Flow Analysis

Network security analysts gather data from diverse sources, from high-level summaries of network flow and traffic volumes to low-level details such as service logs from servers and the contents of individual packets. They validate and check this data against traffic patterns and historical indicators of compromise. Based on the results of this analysis, a decision is made to either automatically manage the traffic or report it to an analyst for further investigation. Unfortunately, due rapidly increasing traffic volumes, there are far more events to check than operational teams can handle for effective forensic analysis. However, just as packets are grouped into flows that share a commonality, we argue that a high-level construct for grouping network flows into a set a flows that share a hypothesis is needed to significantly improve the quality of operational network response by increasing Events Per Analysts Hour (EPAH). In this paper, we propose a formalism for describing a superflow construct, which we characterize as an aggregation of one or more flows based on an analyst-specific hypothesis about traffic behavior. We demonstrate simple superflow constructions and representations, and perform a case study to explain how the formalism can be used to reduce the volume of data for forensic analysis.

==> main-old.tex <==
% HotNETS 2023: https://conferences.sigcomm.org/hotnets/2023/
% CFP: TBD.
% Due: 30 June 2023?
% 6 pages + references?

%\documentclass{hotnets22}

\input{src/preamble.tex}

\title{Superflows: A New Tool for Forensic Network Flow Analysis}
% Mike suggested: Flow graphs, instead
\author{
Authors Blinded
%  Michael Collins\thanks{Authors in alphabetical order} \and
%  Jyotirmoy V. Deshmukh \and
%  Dristi Dinesh \and
%  Mukund Raghothaman \and
%  Srivatsan Ravi \and
%  Yuan Xia
}

\begin{document}

\maketitle

\input{src/abstract.tex} \mclearpage
\input{src/intro.tex} \mclearpage
\input{src/related.tex} \mclearpage
\input{src/sf.tex} \mclearpage
\input{src/studies.tex} \mclearpage
\input{src/future.tex}

%\clearpage
\bibliographystyle{abbrv}
%\begin{small}
\bibliography{src/references}
%\end{small}

% \clearpage
% \appendix
% \input{src/shunt.tex}

\end{document} 


==> src/exp_synth.tex <==
\section{Experimental Superflow Generation}
In order to explore the superflow concept, we have created traffic traces on a Merge testbed using different client/server and service combinations in isolation.  By creating clean traces focusing exclusively on specific classes of traffic, we can examine the construction and description of superflows and determine which attributes are necessary for effectively describing the superflow.  For this work, we have considered three scenarios: {\em scanning}, a {\em modern website} and an {\em ICMP scan and response}.

Scanning, systematically targeting open ports on a network in order to determine the presence of vulnerable services, is an excellent target for a superflow formulation due to the disproportionate footprint scans leave in network traffic summaries.  Scans consist of a large number of packets with slightly different addresses, meaning that a small scan (256 hosts) may take up hundreds of more records than a long, multi-terabyte, data transfer.  

By a {\em modern website}, we mean a website which fetches a multimedia page that requires support information from multiple subsidiary servers.  Examples of such servers include images, multimedia data, advertising, user tracking and JavaScript.  Modern webpages are often comprised of fetches from dozens or hundreds of different websites.  For our initial experiments, we created a network comprised of one root server, and three subsidiary servers which are fetched randomly.   

By {\em ICMP scan and response} we mean a variation on scanning involving multiple protocols.  Scanning, as conceived in the original experiments, is a TCP Half open scan which sends and receives TCP packets.  The ICMP variant scans a network from a hop away and 

==> src/shunt.tex <==
\section{Shunt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{defn}[Packet]
A tuple consisting of fields: $(\src_\ip, \allowbreak \src_\port, \dst_\ip, \dst_\port, t_i, \dots)$. Function
$\timestamp$ maps the packet to $t_i$.
\end{defn}

\begin{defn}[Identically Addressed Packets]
Same source and destination IPs.
\end{defn}

\begin{defn}[Flow]
An ordered sequence of identically addressed packets,  $-\timestamp(\pkt_i)+\timestamp(\pkt_{i+1}) < \mathrm{timeout}$.
\end{defn}

\begin{defn}[Hypothesis class]
% TODO: ???
\end{defn}

\begin{defn}[Superflow]
A collection of flows that share a  common relationship.

Stochastic relationships between flows.
\end{defn}

Examples of superflows:
\begin{enumerate}
\item Bidirectional flow
\item Below here are new things:
\item Webpage Fetch
\item Scan
\item ICMP
\item Print page
\item Torrent
\item IoT?
\item Worm propagation
\item DDoS
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Fodder for Paper 1}

Let $S$ be a set of superflows.
\begin{defn}[Confounder]
A function $f : S \to S$ is a confounder with respect to a property $\varphi:S\to \reals$ if  $\exists s\in S:
\varphi(f(s)) \neq \varphi(s)$.
\end{defn}
